Budget-aware Query Tuning: An AutoML Perspective

Modern database systems rely on cost-based query optimizers to come up with good execution plans for input queries. Such query optimizers rely on cost models to estimate the costs of candidate query execution plans. A cost model represents a function from a set of cost units to query execution cost, where each cost unit specifies the unit cost of executing a certain type of query processing operation (such as table scan or join). These cost units are traditionally viewed as constants, whose values only depend on the platform configuration where the database system runs on top of but are invariant for queries processed by the database system. In this paper, we challenge this classic view by thinking of these cost units as variables instead. We show that, by varying the cost-unit values one can obtain query plans that significantly outperform the default query plans returned by the query optimizer when viewing the cost units as constants. We term this cost-unit tuning process "query tuning" (QT) and show that it is similar to the well-known hyper-parameter optimization (HPO) problem in AutoML. As a result, any state-of-the-art HPO technologies can be applied to QT. We study the QT problem in the context of anytime tuning, which is desirable in practice by constraining the total time spent on QT within a given budget -- we call this problem budget-aware query tuning. We further extend our study from tuning a single query to tuning a workload with multiple queries, and we call this generalized problem budget-aware workload tuning (WT), which aims for minimizing the execution time of the entire workload. WT is more challenging as one needs to further prioritize individual query tuning within the given time budget. We propose solutions to both QT and WT and experimental evaluation using both benchmark and real workloads demonstrates the efficacy of our proposed solutions.

==> backup.tex <==
\begin{figure*}
\centering
\subfigure[\textbf{JOB}]{ \label{fig:query-tuning:impr:job}
    \includegraphics[width=\textwidth]{figures/query-tuning/job-per-query-impr.eps}}
\subfigure[\textbf{Real-A}]{ \label{fig:query-tuning:impr:real-A}
\includegraphics[width=\textwidth]{figures/query-tuning/real-A-per-query-impr.eps}}
\subfigure[\textbf{Real-B}]{ \label{fig:query-tuning:impr:real-B}
\includegraphics[width=\textwidth]{figures/query-tuning/real-B-per-query-impr.eps}}
\vspace{-1em}
\caption{Percentage improvement of the execution time of the best plan found by query tuning (with 100 trials of random search) vs. default plan.}
\label{fig:query-tuning:impr}
%\vspace{-1em}
\end{figure*}

\begin{figure*}
\centering
\subfigure[\textbf{JOB}]{ \label{fig:query-tuning:time:job}
    \includegraphics[width=\textwidth]{figures/query-tuning/job-per-query-time.eps}}
\subfigure[\textbf{Real-A}]{ \label{fig:query-tuning:time:real-A}
\includegraphics[width=\textwidth]{figures/query-tuning/real-A-per-query-time.eps}}
\subfigure[\textbf{Real-B}]{ \label{fig:query-tuning:time:real-B}
\includegraphics[width=\textwidth]{figures/query-tuning/real-B-per-query-time.eps}}
\vspace{-1em}
\caption{Execution time of default plan vs. best plan found by query tuning with 100 trials of random search.}
\label{fig:query-tuning:time}
%\vspace{-1em}
\end{figure*}

\ww{Feedback from Vivek: (1) How do you position this work? It seems as re-purposing the cost model. That is, we are not trying to improve the accuracy of the cost model. Rather, we think of those cost units as another set of knobs and use them to influence the query optimizer. This is similar to query hinting. The difference is that query hinting impacts the query optimizer by restricting the search space, whereas our approach impacts the query optimizer by varying the cost estimation.
(2) What are the baselines to compare against? One baseline is to calibrate the cost units (either for each workload or for each hardware platform). This is necessary to establish the hypothesis/motivation that query-level tuning is useful.
Other baselines include comparing against other query-level tuning techniques, such as query hinting and using cardinality feedback.
}

\ww{Note on calibration and using cardinality feedback: These techniques try to fix the \emph{inputs} to the cost model, with the implicit hypothesis that the cost model itself is accurate. In reality, the cost model is often inaccurate, as it basically consists of cost functions formulated by the cost model designers.
If the cost model is inaccurate (i.e., the cost functions/formulas are inaccurate) for a query, then fixing the inputs cannot make the cost estimates accurate. 
Our technique implicitly assumes that the cost model is not perfect and tries to get the best out of this imperfection. Just like in ML, all models are wrong, but some are useful.}

\ww{Another problem is which cost units should be tuned. SQL Server has around 50 cost units, and tuning all of them may make the search space too large. We currently hand-picked some cost units in our preliminary evaluation, which is not great.}

\ww{Feedback from Bailu: (1) Query hinting can be a baseline (e.g., for the Dynamics workload). (2) The template-based scenario needs more clarity. In the query hinting case, it is unclear how to specify a query hint for a template. It therefore makes more sense to focus on the case of tuning a single query instance.}

\ww{Thoughts on the single-query tuning problem: (1) In our current experiments, we have to specify a search space, which is pretty artificial. (2) We need to think about which cost units should be tuned for a given query. One idea could be to look at the initial plan of the query and find important operators such that tuning their cost units may have impact. (3) We also need to think about the search space of these cost units, i.e., for each cost unit, what should be the range that the search should focus on. (4) The budget allocation problem remains in the case of single-query tuning, i.e., we need to think about how to allocate time to each cost unit or query plan.}

\begin{itemize}
    \item Query tuning aims for finding the best query plan (in terms of some performance metric such as query execution time).
    \item The tuning is performed offline and the tuning time is usually considered a one-shot overhead~\cite{HerodotouB10}.
    \item In practice, however, the tuning time cannot be infinite and must be constrained. In other words, one would desire an \emph{anytime} property~\cite{dta} of query tuning such that, given a constraint or budget on tuning time, return the best query plan found in that time span.
    \item There has been work on query tuning that in particular uses cardinality feedback~\cite{HerodotouB10}.
    This is reasonable, as cardinality estimation error is deemed as one major reason of getting suboptimal query plans~\cite{Lohman-critique}. However, getting cardinality feedback itself is very expensive, and having mixed (both ground-truth and estimated) cardinality often results in inconsistency issues that further mislead the query optimizer~\cite{MarklHKMST07}.
    \item In this work, we take a different route for anytime query tuning by looking into the other aspect of the cost model used by query optimizer, namely, the \emph{cost units} that deemed as constants by the cost model that represent unit cost of CPU or I/O operation~\cite{WuCZTHN13}. As was pointed in previous work~\cite{WuCZTHN13,WuCHN13,WuWHN14,WuNS16}, calibrating these cost units towards the hardware platform where the database server runs on top of often improves the query plan obtained. Nonetheless, the classic view in the literature remains treating these cost units as \emph{constants}, and the calibration procedure is typically done once per platform to make these constants more accurate. As was witnessed in previous work~\cite{WuCZTHN13}, there are often variances when calibrating these cost units using different queries, which indicates that they may not be ``constants'' per se.
    \item In this paper, we take a different view by thinking of these cost units as \emph{tunable} variables or parameters, which means that they can be different for each different query. Our goal is then to find the best cost units that result in the minimum execution time of a given query. This is similar to the \emph{hyperparameter optimization} (HPO) problem that has been studied intensively in the machine learning (ML) literature.
    One can think of a query as an ML model in the HPO context, though the goal of HPO is to find the best HP configuration that leads to the highest model quality (in terms of e.g., accuracy, AUC score, etc.).
    \item Although the single-query cost model tuning problem is very similar to the HPO problem, in practice one often wants to tune an entire workload with multiple queries. This creates a new research problem when a budget on the tuning time is given as a constraint. Existing budget-aware HPO approaches, such as Hyperband~\cite{Hyperband}, BOHB~\cite{BOHB}, CFO~\cite{CFO}, and BlendSearch~\cite{BlendSearch}, only deal with HPO for a single ML model and cannot be directly used for workload-level tuning. We formulate the budget-constrained/anytime workload-level tuning problem and propose new solutions.
\end{itemize}
